Generalized Whac-a-Mole

We consider online competitive algorithms for the problem of collecting weighted items from a dynamic set S, when items are added to or deleted from S over time. The objective is to maximize the total weight of collected items. We study the general version, as well as variants with various restrictions, including the following: the uniform case, when all items have the same weight, the decremental sets, when all items are present at the beginning and only deletion operations are allowed, and dynamic queues, where the dynamic set is ordered and only its prefixes can be deleted (with no restriction on insertions). The dynamic queue case is a generalization of bounded-delay packet scheduling (also referred to as buffer management). We present several upper and lower bounds on the competitive ratio for these variants.

==> dynamic_sets_rand_upper.tex <==
% marek, Feb 6, 2008

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DECREMENTAL UNIFORM SETS, RANDOMIZED UPPER BOUND
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We present a simple randomized algorithm with competitive ratio $\e/(\e-1)$,
thus matching the lower bound from the previous section.

%%%%%%

\myparagraph{Algorithm~{\UniRand}}.
At each step collect with equal probability one of the pending items.

\smallskip

The idea behind the competitive analysis is to
prove first that the optimal strategy of the adversary can be easily described:
without loss of generality, at each step the adversary
collects one item and deletes the same item. Then we analyze the
competitive ratio of {\UniRand} against such an adversary.

The number of items in the initial set is denoted by $n$. By
$a$ we denote the number of active items at a given step,
and by $p\le a$ the number of pending items. Note that
$p$ is a random variable. We consider states of the game
conditioned on $p$ being fixed, and we refer to such a state
as a \emph{configuration $(a,p)$}.  The definition
of {\UniRand} implies that in a configuration $(a,p)$
each active item is pending with  probability $p/a$.

We analyze the relation between the gain of {\UniRand} and
that of the adversary starting from each fixed
configuration $(a,p)$.
%We can assume that the
%adversary always collects an item, if there is one pending.
Since the items are identical
and the algorithm's pending items are distributed
uniformly, we need not specify which items are
deleted by the adversary in a given step, only their
quantity.

We can split these steps into smaller parts---an \emph{elementary}
step consists in either collecting an item or deleting an item.
We can thus describe the adversary's strategy as a sequence
$S \in \{\dele,\take \}^*$, where $\take$ means that the adversary
takes an item (and allows the algorithm to take one as well)
and $\dele$ means that the adversary deletes an item.
Not all such sequences are feasible. In the following we consider
only the \emph{feasible} strategies $S$ for configuration $(a,p)$,
i.e. those in which:
(i) the number of $\dele$ operations in $S$ is $a$,
(ii) in every suffix of $S$ the number of $\take$ operations is
not greater than $\dele$ operations.


By $E_{a,p}[S]$ we denote the expected gain of
Algorithm~{\UniRand} starting from configuration $(a,p)$,
versus adversary strategy $S$.

%%%%%%%%%

\begin{lemma}\label{lem: E_ap monotone with p}
For every $a,p,S$, it holds that $E_{a,p+1}[S] \geq E_{a,p}[S]$.
\end{lemma}

\begin{proof}
We prove the inequality by induction on pairs $(p,S)$,
where $(p_1,S_1)<(p_2,S_2)$ if $|S_1| \leq |S_2|$
$|S_1| = |S_2|$ and $p_1<p_2$.
The inductive basis is straightforward:
if $S=\dele^a$ then $E_{a,p+1}[\dele^a] = 0 = E_{a,p}[\dele^a]$.
If $p=0$ then clearly $E_{a,1}[S] \geq 0 = E_{a,0}[S]$.

In the inductive step, we have two cases depending on
the first action of $S$. If $S=\take S'$, then
$E_{a,p+1}[\take S']=1+E_{a,p}[S'] \geq 1+E_{a,p-1}[S']=E_{a,p}[\take S']$,
by the inductive assumption.
If $S=\dele S'$, since we have $p+1$ pending items,
the adversary deletes a pending item
with probability $\frac{p+1}{a}$ and a non-pending item with
probability $\frac{a-p-1}{a}$. Using the inductive assumption, we get
%
\begin{eqnarray*}
E_{a,p+1}[\dele S'] &= &
 	\frac{a-p-1}{a} E_{a-1,p+1}[S'] + \frac{p+1}{a} E_{a-1,p}[S']
				\\
	&\geq & \frac{a-p-1}{a} E_{a-1,p}[S'] +
		\brackd{ \frac{1}{a} E_{a-1,p}[S'] + \frac {p}{a}E_{a-1,p-1}[S'] }
			\;= \; E_{a,p}[\dele S'],
\end{eqnarray*}
%
%%% Commented out, might be useful later on %%%
\begin{comment}
We prove the second inequality by the induction on pairs $(S,p)$ as well.
If $p=0$ then clearly $E_{a+1,0}[Sd] = 0 = E_{a,0}[S]$. If $S=d^a$ then
$E_{a+1,p}[d^ad] = 0 = E_{a+1,p}[d^a]$. This proves the induction basis.
For the induction step consider first $S=tS'$:
$E_{a+2,p}[tS'd]=1+E_{a+1,p}[S'd] \geqslant 1+E_{a,p-1}[S']=E_{a,p-1}[\take S']$.
If $S=dS'$ we again use the fact that the pending items are distributed uniformly among the
active items:
\begin{align*}
E_{a+1,p}[dS'd]=1 + \frac {a-p+1}{a+1}E_{a,p}[S'd] + \frac {p}{a+1}E_{a,p-1}[S'd]\\
E_{a,p}[dS']=1 + \frac {a-p}{a}E_{a,p}[S'] + \frac {p}{a}E_{a-1,p-1}[S']
\end{align*}
Multiplying by $a(a+1)$ and subtracting
\begin{multline*}
a(a+1)(E_{a+1,p}[dS'd] - E_{a,p}[dS']) = \\
a(a-p+1)E_{a,p}[S'd] + ap E_{a,p-1}[S'd]
- (a+1)(a-p)E_{a-1,p}[S'] - (a+1)(p) E_{a-1,p-1}[S']
=\\
(a+1)(a-p)(E_{a,p}[S'd] - E_{a-1,p}[S']) + (a-1)p(E_{a,p-1}[S'd] - E_{a-1,p-1}[S'])
+E_{a,p}[S'd] -  E_{a-1,p-1}[S']
 \geqslant\\
 E_{a,p}[S'd] -  E_{a-1,p-1}[S'] \geqslant
 E_{a,p-1}[S'd] -  E_{a-1,p-1}[S'] \geqslant 0
\end{multline*}
Which proves the inductive step.
\end{comment}
%%% End of commented out text %%%
\qed
\end{proof}

\begin{lemma}\label{lemma:td_inversing}
Let $S=S_1\take \dele S_2$ be a feasible strategy for $(a,p)$.
If $S'=S_1\dele \take S_2$ is also a feasible strategy, then
$E_{a,p}[S] \geq E_{a,p}[S']$.
\end{lemma}

\begin{proof}
Suppose first that $S=\take \dele S_2$.
If $p=0$ then the claim is obvious, as $E_{a,0}[S]=E_{a,0}[S']=0$, and
if $p=1$ then $E_{a,1}[S]=1 \geq E_{a,1}[S']$.
So consider $p>1$. By direct calculation:
%
\begin{eqnarray*}
E_{a,p}[\take \dele S_2]
	&=&  1+E_{a,p-1}[\dele S_2]
			\\
	&=&  1+\frac{a-p+1}{a} E_{a-1,p-1}[S_2]+ \frac{p-1}{a} E_{a-1,p-2}[S_2]
			\\
	&=&  1+\frac{a-p}{a} E_{a-1,p-1}[S_2]+ \frac{1}{a} E_{a-1,p-1}[S_2]
			+ \frac{p-1}{a} E_{a-1,p-2}[S_2]
			\\
	&\geq&  1+\frac{a-p}{a} E_{a-1,p-1}[S_2]+ \frac{1}{a} E_{a-1,p-2}[S_2]
	 					+ \frac{p-1}{a} E_{a-1,p-2}[S_2]
			\\
	&=& 1+\frac{a-p}{a} E_{a-1,p-1}[S_2]+ \frac{p}{a} E_{a-1,p-2}[S_2]
	 		\\
	&=& \frac{a-p}{a} E_{a-1,p}[\take S_2]+ \frac{p}{a} E_{a-1,p-1}[\take S_2]
			\\
	&=& E_{a,p}[\dele\take S_2] \enspace.
\end{eqnarray*}
%
Now consider the general case, when $S=S_1\take\dele S_2$ and $S'=S_1\dele\take S_2$. Then
%
\begin{align*}
E_{a,p}[S] \;=\; E_{a,p}[S_1\take\dele S_2]
			\;=\; \sum_i c_i E_{a-k,p-i}[\take\dele S_2]
	\\
E_{a,p}[S'] \;=\; E_{a,p}[S_1\dele \take S_2]
		\;=\; \sum_i c_i E_{a-k,p-i}[\dele\take S_2]
\end{align*}
%
for some $k$, $\{c_i\}$. By the previous calculations for all $i$,
$E_{a-k,p-i}[\take\dele S_2] \geq E_{a-k,p-i}[\dele\take S_2]$
and hence
%
\begin{eqnarray*}
E_{a,p}[S] \;=\; E_{a,p}[S_1\take\dele S_2]
			&=& \sum_i c_i E_{a-k,p-i}[\take\dele S_2] \\
			&\geq& \sum_i c_i E_{a-k,p-i}[\dele\take S_2]
			\;=\; E_{a,p}[S_1\dele\take S_2]
			\;=\; E_{a,p}[S'],
\end{eqnarray*}
%
completing the proof.
\qed
\end{proof}

We say that a strategy $S$ for $(a,a)$ is a \emph{$k$-strategy}
if it collects $k$ items.
Let $N_a=(\take\dele)^a$ define the \emph{natural} strategy for configuration $(a,a)$, i.e. the one in which in each step we take an item and then delete
it. The following lemma shows that any $k$-strategy for $(a,a)$ is, in a
sense, dominated by $N_k$ on $(k,k)$.
%
\begin{lemma}\label{lemma:k_optimal_strategy}
Let $S$ be a $k$-strategy for $(a,a)$. Then
$E_{a,a}[S] \geq E_{k,k}[N_k]$.
\end{lemma}

\begin{proof}
We apply Lemma \ref{lemma:td_inversing}. We know that in $S$ there are $k$
operations $\take$. Let $p_1 > p_2 > \ldots > p_k$ be their positions (counting
from the right). As $S$ is feasible then no suffix contains more $\take$
operations than $\dele$
operations, hence $p_i \geq 2i$. We iteratively modify $S$ so that
in the end in $S$ one has $p_i=2i$. Consider $p_i$ for $i=1 ,\ldots , k$. Suppose
$p_i >2i$. As $p_{i-1} = 2i-2$ there are only $\dele$ operations on positions
$2i,2i+1,\ldots , p_i - 1$. Then by Lemma~\ref{lemma:td_inversing}
we can move $\take$ operation from position $p_i$ to position $2i$ by
consecutively inverting it with $\dele$ operations. The value of $E_{a,a}[S]$
cannot increase by Lemma \ref{lemma:td_inversing}.

After ending the process we obtain another $k$-strategy $S'=\dele^{a-k}(\take\dele)^k$
and $E_{a,a}[S] \geq E_{a,a}[S']$. Clearly
$E_{a,a}[\dele^{a-k}(\take\dele)^k]=E_{k,k}[(\take\dele)^k]=E_{k,k}[N_k]$.
\qed
\end{proof}

We prove that the competitive ratio of the
Algorithm~{\UniRand} is at most $\e/(\e-1)$.

%%%%%%%%%%%

\begin{lemma}\label{lemma:upper_bound_estimation}
For any integers $p \leq a$, it holds that
$E_{a,p}[(\take\dele)^a] \geq a(1-(1 - 1/a)^p)$.
\end{lemma}

\begin{proof}
For $p = 0,1$, $E_{a,p}[(\take\dele)^a] = p$ and the lemma trivially holds.
Also if $a = p = 2$, then
$E_{a,p}[(\take\dele)^a] = 3/2 = a(1-(1 -1/a)^p)$ .

For the remaining values of $a$ and $p$ we prove the lemma by induction on $a$.
We note that for $p \geq 2$
$$
E_{a,p}[(\take\dele)^a] \;=\;
 		\frac{a-p+1}{a} E_{a-1,p-1}[(\take\dele)^{a-1}]
				+ \frac{p-1}{a} E_{a-1,p-2}[(\take\dele)^{a-1}] + 1 \enspace,
$$
as the pending items are distributed uniformly among active items.
Note that this is the same recurrence as in the proof of the lower bound.
Thus, using the induction assumption, we get
%
\begin{eqnarray*}
	E_{a,p}[(\take\dele)^a]
		&\geq
			&\frac{a-p+1}{a} \left(a-1\right)\left(1-\left(\frac {a-2}{a-1}\right)^{p-1}\right)
			+ \frac{p-1}{a} \left(a-1\right)\left(1-\left(\frac {a-2}{a-1}\right)^{p-2}\right)
			+ 1
			\\
	&=&
		a - \frac{(a-1)^2}{a} \left(\frac {a-2}{a-1}\right)^{p-2}
				\left(1 + \frac{p-2}{(a-1)^2} \right)
			\\
	&\geq&
		a - \frac{(a-1)^2 }{a}\left(\frac {a-2}{a-1}\right)^{p-2}
			\left(1 + \frac{1}{(a-1)^2} \right)^{p-2}
		 \\
	&\geq&
	 	a - \frac{(a-1)^2}{a} \left(\frac {a-1}{a}\right)^{p-2}
		\\
	&=&  a \left(1 - \left(\frac {a-1} a \right)^p\right),
\end{eqnarray*}
%
completing the proof.
\qed
\end{proof}

\begin{theorem}
Algorithm {\UniRand} is $\e/(\e-1)$-competitive.
\end{theorem}

\begin{proof}
Let $k$ be the number of items collected by the adversary from $n$ elements.
Consider any $k$-strategy $S$ for $(n,n)$.
By Lemmas~\ref{lemma:k_optimal_strategy},\ref{lemma:upper_bound_estimation},
$E_{n,n}[S] \geq E_{k,k}[(\take\dele)^k]
	\geq k (1 - (1-1/k)^k)$.
Therefore, the competitive ratio is at most
$$
\frac k {E_{n,n}[S]}  \;\leq\;
  		\brackd{1 - \left(1 - \frac {1}{k}\right)^k }^{-1}
			\;<\;   \frac {\e} {\e-1} \enspace,
$$
\qed
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

